LASER: A Neuro-Symbolic Framework for Learning Spatial-Temporal Scene Graphs with Weak Supervision

Supervised approaches for learning spatio-temporal scene graphs (STSG) from video are greatly hindered due to their reliance on STSG-annotated videos, which are labor-intensive to construct at scale. Is it feasible to instead use readily available video captions as weak supervision? To address this question, we propose LASER, a neuro-symbolic framework to enable training STSG generators using only video captions. LASER employs large language models to first extract logical specifications with rich spatio-temporal semantic information from video captions. LASER then trains the underlying STSG generator to align the predicted STSG with the specification. The alignment algorithm overcomes the challenges of weak supervision by leveraging a differentiable symbolic reasoner and using a combination of contrastive, temporal, and semantics losses. The overall approach efficiently trains low-level perception models to extract a fine-grained STSG that conforms to the video caption. In doing so, it enables a novel methodology for learning STSGs without tedious annotations. We evaluate our method on three video datasets: OpenPVSG, 20BN, and MUGEN. Our approach demonstrates substantial improvements over fully-supervised baselines, achieving a unary predicate prediction accuracy of 27.78% (+12.65%) and a binary recall@5 of 0.42 (+0.22) on OpenPVSG. Additionally, LASER exceeds baselines by 7% on 20BN and 5.2% on MUGEN in terms of overall predicate prediction accuracy.

==> figures/datalog_implementation.tex <==

\begin{lstlisting}[language=scallop,numbers=none,xleftmargin=.05\textwidth]
// Basic types
type Var = String
type Obj = u32
type Time = u32

//////////////////////////
// Variable assignments //
//////////////////////////
type variable(Var)
type object(Obj)
rel var_obj = disjunct[v](o: variable(v) and object(o))
type name(o: Obj, name: Var)

//////////////////////////////////
// Spatial-temporal scene graph //
//////////////////////////////////
type time(time: Time)
type max_time(time: Time)
type sg_unary_atom(predicate: String, fid: Time, o1: Obj)
type sg_binary_atom(predicate: String, fid: Time, o1: Obj, o2: Obj)

///////////////////////////////////
// Specification on scene graphs //
///////////////////////////////////

// Term: either constant string or variable
type Term = Const(String) | Var(Var)

// TForm: temporal formula, containing `Global`, `Finally`, `Until`,
// and `Next`
type TForm = Global(TForm) 
            | Finally(TForm) 
            | Until(TForm, TForm) 
            | Next(TForm) 
            | Logic(LForm)

// LForm: logical formula, containing logical conjunction and atomic
// queries
type LForm = And(LForm, LForm) 
            | Unary(String, Term) 
            | Binary(String, Term, Term) 
            | NegUnary(String, Term) 
            | NegBinary(String, Term, Term) 

// The specification
type spec(psi: TForm)

// Aligning logical formula: the formula `phi` is aligned with the scene
// graph starting from time `s`, given the variable assignment `va`
type align_lform(phi: LForm, s: Time)
rel align_lform(phi, s) = case phi is And(l, r) and align_lform(l, s) 
and align_lform(r, s)

rel align_lform(phi, s) = case phi is Unary(pred, Var(var)) 
    and var_obj(var, o) and sg_unary_atom(pred, s, o) and time(s)
                        
rel align_lform(phi, s) = case phi is Unary(pred, Const(c)) 
    and var_obj(var, o) and has_constant(pred, s, c) and time(s)

rel align_lform(phi, s) = case phi is NegUnary(pred, Var(var)) 
    and var_obj(var, o) and not sg_unary_atom(pred, s, o) and time(s)

rel align_lform(phi, s) = case phi is NegUnary(pred, Const(c)) 
    and var_obj(var, o) and not has_constant(pred, s, c) and time(s)

rel align_lform(phi, s) = case phi is Binary(pred, Var(v1), Var(v2))
    and var_obj(v1, o1) and var_obj(v2, o2) 
    and sg_binary_atom(pred, s, o1, o2) and time(s)

rel align_lform(phi, s) = case phi is Binary(pred, Var(v1), Const(c2))
    and var_obj(v1, o1) and name(o2, c2) 
    and sg_binary_atom(pred, s, o1, o2) and time(s)

rel align_lform(phi, s) = case phi is Binary(pred, Const(c1), Var(v2))
    and name(o1, c1) and var_obj(v2, o2) 
    and sg_binary_atom(pred, s, o1, o2) and time(s)
                          
rel align_lform(phi, s) = case phi is Binary(pred, Const(c1), Const(c2)) 
    and name(o1, c1) and name(o2, c2) 
    and sg_binary_atom(pred,s, o1, o2) and time(s)

rel align_lform(phi, s) = case phi is NegBinary(pred, Var(v1), Var(v2)) 
    and var_obj(v1, o1) and var_obj(v2, o2) 
    and not sg_binary_atom(pred, s, o1, o2) and time(s)

rel align_lform(phi, s) = case phi is NegBinary(pred, Var(v1), Const(c2)) 
    and var_obj(v1, o1) and name(o2, c2) 
    and not sg_binary_atom(pred, s, o1, o2) and time(s)

rel align_lform(phi, s) = case phi is NegBinary(pred, Const(c1), Var(v2)) 
    and name(o1, c1)  and var_obj(v2, o2) 
    and not sg_binary_atom(pred, s, o1, o2) and time(s)

rel align_lform(phi, s) = case phi is NegBinary(pred, Const(c1), Const(c2)) 
    and name(o1, c1) and name(o2, c2) 
    and not sg_binary_atom(pred, s, o1, o2) and time(s)

// Aligning temporal formula: the formula `psi` is aligned with 
// the scene graph starting from time `s`,  
// given the variable assignment `va`
type align_tform(psi: TForm, s: Time)
rel align_tform(psi, s) = case psi is Global(p1) and max_time(n) 
                          and align_all_tform(p1, s, n)
rel align_tform(psi, s) = case psi is Finally(p1)
                          and align_once_tform(p1, s)
rel align_tform(psi, s) = case psi is Until(p1, p2) 
                          and time(t + 1) and s < (t + 1) 
                          and align_all_tform(p1, s, t) 
                          and align_tform(p2, t + 1)
rel align_tform(psi, s) = case psi is Until(p1, p2) 
                          and align_tform(p2, s)
rel align_tform(psi, s) = case psi is Next(p1) 
                          and align_tform(p1, s + 1) and time(s)
rel align_tform(psi, s) = case psi is Logic(p1) and align_lform(p1, s)

// Helper relations
rel has_constant(pred, fid, constant) = sg_unary_atom(pred, fid, o)
                                        and name(o, constant)
type align_once_tform(psi: TForm, s: Time)
rel align_once_tform(psi, s) = align_tform(psi, s)
rel align_once_tform(psi, s) = align_once_tform(psi, s + 1) 
                               and time(s)
type align_all_tform(psi: TForm, s: Time, t: Time)
rel align_all_tform(psi, s, s) = align_tform(psi, s)
rel align_all_tform(psi, s, n + 1) = align_all_tform(psi, s, n) 
                                    and align_tform(psi, n + 1) 
                                    and time(n + 1)

///////////////////////////
// Solving for alignment //
///////////////////////////
rel aligned() = spec(psi) and align_tform(psi, 0)

///////////////////////////
//     Temporal Loss     //
///////////////////////////
rel temporal_diff(t_post - t_pre) = spec(psi) and align_tform(psi, 0)      and case psi is Until(Finally(pre), Finally(post)) 
    and align_tform(pre, t_pre) 
    and align_tform(post, t_post) 
    and t_post > t_pre

\end{lstlisting}
\label{fig:dl_implementation_2}



\begin{table}
\begin{tabular}{c|l|cc}
\toprule
\hline
\textbf{Supervision} & \textbf{Method} & \textbf{Unary Accuracy (\%)}  & \textbf{Binary Accuracy(\%)}    \\ \hline
\multirow{2}{*}{No supervision} & SIGLIP & 20.41 & 62.41 \\
& Random & 17.10 & 27.86 \\ \hline
\multirow{3}{*}{Fully supervised} & IPS-Transformer & 14.67 &  \textbf{74.75} \\ 
& VPS-Transformer & 5.46 &  64.8 \\
& TEMPURA & 11.90 & 9.81 \\ 
\hline
Weakly supervised & \ours & \textbf{31.64} & \textbf{70.12} \\ 
\hline
\bottomrule
\end{tabular}
\end{table}
